Inverting the Kohn-Sham equations with physics-informed machine learning

Electronic structure theory calculations offer an understanding of matter at the quantum level, complementing experimental studies in materials science and chemistry. One of the most widely used methods, density functional theory (DFT), maps a set of real interacting electrons to a set of fictitious non-interacting electrons that share the same probability density. Ensuring that the density remains the same depends on the exchange-correlation (XC) energy and, by a derivative, the XC potential. Inversions provide a method to obtain exact XC potentials from target electronic densities, in hopes of gaining insights into accuracy-boosting approximations. Neural networks provide a new avenue to perform inversions by learning the mapping from density to potential. In this work, we learn this mapping using physics-informed machine learning (PIML) methods, namely physics informed neural networks (PINNs) and Fourier neural operators (FNOs). We demonstrate the capabilities of these two methods on a dataset of one-dimensional atomic and molecular models. The capabilities of each approach are discussed in conjunction with this proof-of-concept presentation. The primary finding of our investigation is that the combination of both approaches has the greatest potential for inverting the Kohn-Sham equations at scale.

==> comments_from_main.tex <==
% This work serves as a proof of concept. Improvement is possible in many ways. \textcolor{red}{is it?} Convolutions provide the network a way to learn about non-localtiy of the density but have multiple drawbacks. The use of convolutions is not spatial-invariant. The network is initialized with a set kernel for each convolution and when moving to a new grid the kernel won't change but the spacing between the points will.
% One method of interest for learning KS potentials in a grid invariant manner is through neural operators. Specifically Fourier neural operators. This would allow the network to learn in Fourier space but it moves away from the idea of non-locality and changes the focus to frequency. \textcolor{red}{graph neural network?}
% The fact that the network is employing exact KS eigenfunctions within it's loss function is an issue to be addressed. If the future goal of the network is to predict exact XC potentials for complicated densities there won't be a set of exact KS eigenfunctions to employ. Thus the network will need to extrapolate a large distance outside of its training set, which is extremely unfavorable given the nature of machine learning. If there was a way to train a network to decompse an electronic density into exact KS eigenfunctions that might be employed. Another idea is exchanging the KS equations for the Levy Perdew Sahni (LPS) equation and trying to predict Exchange Correlation Pauli (XCP) potnetials.
% This work try's to predict the exact KS potnetial as a whole but it would be interesting to have the network predict solely the XC potential since the Hartree and external potentials are already known exactly.

%  There are already multiple plans for the expansion and application of this work. As previously stated inversions of electronic densities with neural networks has already been a topic of research for many. While the application of a PINNs framework to an inversion network is a novel idea there is another avenue of interesting research for this work. Exchanging the KS equation as the training function of the neural network for the Levy-Perdew-Sahni equation. Doing this should enable the network to learn the mapping between the electronic density and KS potential plus one new term, the Pauli potential. 

%   Convolutions are immensely common in the field of image processing. Networks learn how to observe characteristic features by optimizing the features that the convolutions identify. Normally there are many convolutions in a single layer in parallel rather than a single set of them in series as in this net. It may be pertinent to think about and explore multiple convolutions for the presented work. rather than working in a single channel it may be best to provide the network with two so that it can provide the network wit information about the left and right sides of the density.

%   There are many different ways to process and examine the shape of a function. In this case convolutions were used to look at values of the density in a region around a single point in space. Over time observing larger non-local regions. Another method that is useful in the field of function transformation is neural operators. 

% While the simple network is able to predict potentials within a simple domain with relatively low mean absolute errors, moving closer to a realistic 1D system saw a significant increase decrease in the networks ability to produce potentials that generate correct eigenvalues. The overall structure of the network needs improvement to be able to learn more complicated domains, especially if the goal is exact KS and by extension XC potentials. 

% Chemical space is complex and spans a wide array of varied and interesting effects. The examples presented above are simplified models of atomic and diatomic systems in one dimension. In three dimensions with many atoms the spacing between points in chemical space can be large or there can be holes. PINNs looks to address this problem through it's greater transferability. In the case of this example, and maybe others, the data-driven neural networkdoes better in the limit of large datasets. But, when reduced to learning on a small set the PINNS should still be able to learn a relatively good approximation across the whole range whereas the data driven networks may fail at different points.

% The dataset size for each single-variable case was 41 potentials. To achieve results anywhere near this with the "fully" varying case the dataset size was 729 potentials and the size of the network much larger. Each of these exactly solvable model systems are one dimensional. Moving to 3D and more complicated systems will call for larger datasets with even thinner density of chemical information. 

% If a system can be defined by a single variable and it is calculated or observed in integer units of that variable, each data point is simply one unit dist apart from its nearest neighbor. With 2 variables each neighbor is 1.404 units apart. Moving to the case where the distance as well as well as the charge of each well is allowed to vary each data point is separated by a distance of 1.73 units. Moving into three dimensions and increasing thew number of atomic wells vastly increases the dimensionality and complexity of the problem that we are trying to learn. It will be easier to train Physics informed neural networks to be transferable across wide ranges of chemical space because of this. 

% If a system can be defined by a single variable it can be discretized into $N$ samples and used to train an neural networkfor prediction. When moving to a system of two variables, to retain a comparable density of data, the number of samples needed is $N^2$. 

% This work exists as a simple proof of concept for the prediction of KS potentials using PINNs. 

% % varying charge

% The exact KS potentials for these systems were acquired through the reverse-engineering function within the iDEA code. \textcolor{red}{ref} The network displays low \% errors for the higher lying eigenvalues of the system. 

% The error in the lowest lying eigenvalue of the system can be attributed to the spacing of the grid that the density was computed on. The network is learning from how well a predicted potential fits a set of KS eigenfunctions, their second derivatives, and eigenvalues. 

% Plotting the MAE of the potentials predicted for this dataset computed on grid of 301 and 501 points demonstrates this idea. 

% The error on the edges of the box are comparable showing that increasing the density of the grid doesn't increase the networks ability to =learn the correct decay of the potential but, the peaks in the center of the plot are quite different. In fact, the error decreased at about the same rate that the density of the grid increased, a factor of around 1.5 for the error and 1.65 for the density of points. The ability to take accurate derivatives of low density information, especially in rapidly varying regimes, is important to improving the accuracy of learning to predict potentials in this manner.

% In this simplified set the eigenvalues shouldn't shift a large amount is the spacing is decreased. On the other hand, the eigenfunctions and especially second derivatives will provide the network more information about the cusps in the potential. Leading the network to be better able to predict potetials for the spectrum of eigenvalues.

% The fact that the higher lying eigenvalues show such small absolute percent errors is encouraging. It shows that the network can learn the proper shape of the potential as it moves to long distances. 

% The mean absolute percent error (MAPE) of each charge value can be calculated and outliers in each can be removed. After doing this, the MAPE for the complete set is calculated to be .189\% which corresponds to errors of .0006 to .0065 Hartree.

% %The network was trained on a dataset with two atomic wells of fixed charge seperated by a distance $d$. The distance between the wells varied between the values of one and five in increments of 0.1. Ten percent of the data was held back for testing and another ten percent was held back for validation. Like the previous example the potentials and densities are represented on a 1D grid that spans the coordinates of [-15,15] in steps of 0.1. 

% %The network appears to perform on this set of potentials just as well as the previous case. With a very similar MAPE of .16\% after outliers are removed. But, the actual eigenvalues of this system are greater in value than that of the single well case. The minimum eigenvalue of the double well case is -.95 Hartree whereas for the single well it is -3.5 Hartree.

% %Given this discrepancy in energy values one might think it is better to report the MAE rather than the MAPE. But, the \% error gives a better idea as to the correctness of the potential relative to the exact potential for each eigenvalue.

% %Why are the \% error so similar when the eigenvalues are this different? If we look at the error between the predicted and exact potentials the differences looks the same for all cases. 

% %the MAPE for this case correspond to and error in Hartree between .0004 and .0013. The mean of this network lies within chemical accuracy.

% %Looking at the cosine similarity of the dataset the potentials of the varying distance set are less similar than the single well case. The stripe of yellow along the main diagonal of the matrix is less broad and doesn't fan out near the tail. Each increment in the distance between two wells creates equally dissimilar potentials. Also, examining the range of values in the plotted reveals the the main diagonal already contains the range of values that are plotted for the single well case. Numerically the minimum cosine similarity value in the off diagonal corners is about .90, .092 less than the single well case. All of this would suggest that the double well case should be more complex than the single well case. But, looking to the absolute percent error of the eigenvalues the networks seem to perform at about the same efficiency. 

% %Something that might explain this is the Euclidean distance of the potentials. The maximum distance between any two potentials in this case is just about 4, around 4.25 times less than the case of the varying well depth. Causing the density inputs to be less varied in overall magnitude making the mapping between the two also easier to learn. There is a trade off happening that leads to the two sets having similar complexity in the case of learning.

% %At this point, if the two sets are similar in complexity why include a second and not just move on to the fully varying dataset? The overall error in the potential are smaller than those present in the varying well depth case. The error at the cusps in the potential where the atomic centers would exist is still present and always underestimates the actual potential. Now though, even though it is less pronounced, the network makes errors when predicting the overlap of the two wells. But, the error isn't consistent like the underestimation at atomic centers. The network over and under predicts the turning point between the two wells. the error itself is also not uniform in location, the error can appear centered on the turning point or on the left or right sides of it. The error will mostly likely reduce if the resolution of the grid is increased but not because the second derivatives are improving. Truly fixing this error comes down to more intelligent architecture design.

% %The reduction in the size of the errors is most likely due to the range of densities that the network need to predict over. Since the depth of the wells are fixed and the only changing variable is the distance between the wells, the peaks of the densities are relatively unchanging in magnitude. The network doesn't have to learn to map a range of different magnitudes of densities to a range of different potential magnitudes. The part of the mapping that is sensitive to small changes. This is showing that it is easier to learn over a set of molecules with many similar atomic centers and density profiles rather than a wide range of molecules with widely varying atomic sizes and density profiles.

% %Training the network with the set of 729 calculations, an optimizaed network is able to achieve potentials with errors between 6.6e-6
% %\% and 6.5\% for predicted eigenvalues. The MAE to identify outliers is 1.65\% and after removing the outliers from the set is 1.5\%.

% %The MAE of each eigenvalue is also calculated and plotted with an error bar of one standard deviation. each of the first five eigenvalues has a MAE that lies below 1.5\% while the sixth lies well above 2\%. 

% %Taking the MAE of each eigenvalue and multiplying them by the correct eigenvalue results in a range of error in Hartree between the values of .005 and .07. The larger error is actually a result of the ground state of the system.

% %It is hard to key into a specific error that the network is making when predicting potentials for this dataset. There are errors across the whole potential rather than just at the the overlap of the two wells or their cusps. More interesting is a comparison of PINN versus its data driven counterpart. 

% %By taking a fixed network architecture and providing it with either a physics informed loss function or a data driven one, the two can be compared. It can be seen that the data driven network performs on average better across the whole potential. Mostly because the predictions of the tails of the potential are much better than PINN. Yet, the PINN has better prediction of eigenvalues and of the lower energy parts of the potential. The error around the well bottoms for both networks have similar max values but the error for the PINN has the same sharp peaks like the single well case.

% %The reason that the data driven network performs better at the tails of the potential is due to the fact that the is learning directly from the difference of potentials. Since the physics informed neural network is learning from the physics of the mapping from density to potential through the KS eigenfunctions. If it were provided with even more higher energy states it would be able to learn the mapping more completely.

% %To inform why one might look to employ PINNs when possible there is a simple constructed example. Using the system described in the following subsection and the network architecture in the one after two neural networks were trained. The dataset had five data points. One networkhad a general data driven structure learning from a difference of the predicted potential and the ground truth. The other is learning from the residual of the KS equation and the KS eigenfunctions which describe the physics of the KS potential. Each network is taking the density which results from the exact potential and trained to predict said potential. When the middle sample is removed from the training set for validation the general networkcannot learn to predict the correct shape of the potential. Demonstrating PINNs ability of interpolation from a minimal dataset or datasets that may have holes in the region it is trying to cover.
% %
% %\begin{figure}[H]
% %    \centering
% %    \includegraphics[scale=.6]{images/dist/PINN_VS_PUNN.png}
% %    \caption{Two neural networks were trained employing the same architecture. The difference is the loss function used to inform the networks learning. Plotted in the image is the validation data point for a data-set of varying well distance. The networkwas trained on a set of well distances where $d=[1,2,4,5]$ and validated where $d=3$. The general networkis a MSE loss of the predicted potential and the validation potential. The PINN is the MSE loss of a vector of zeroes and the residual of the re-arranged KS equation. The training of both networks was stopped when their validation loss had reached the minimum, within a certain number of epochs. The general networkdoes not generalize as well to a set of data as a PINN? This can be seen in it's struggle to predict the potential at one unit d away from the training set, as compared to the PINN.}
% %   \label{fig:PINNvPUNN}
% %\end{figure}

% %At first glance the overall complexity of this dataset might appear minimal. Looking to the cosine similarity of the potentials, the smallest value plotted is about .993 which says that all the functions are almost the same. stopping there would confirm the original conclusion. Yet, it is important to note that small changes in the external potential of the system can cause large changes in the calculated electronic density. More simply, the magnitude of the potentials is also important not just the angle between them in N-dimensional space. The Euclidean distance gives an idea as to the difference in magnitude of all of the potentials in the set. Together these two measures give a more complete image of the difficulty of learning a particular set of potentials.

% There are many exact conditions that exist in DFT that the XC energy or potential functional should display. One of these exact conditions is that the potential should decay at a rate of -1/r as one moves away from the system of interest. This exact condition ensures that as any of the non-interacting electrons moves away it always observes the charge of the ionized system it is leaving. The ionization potential and chemical potential of the system are intrinsically tied to this exact condition. Thus it is important for any inversion method used to be able to recover these tails. But, it is difficult to obtain proper decay of the tails without taking the proper considerations into account\cite{XXX}. We bring this up to make two points. One about PINNs and one about ML for inversions in general.

% The first point is that PINN frameworks are able to learn a more proper shape of the XC potential decay even when learning from KS eignfunctions and eigenvalues that come from improper potentials. This feature is most pronounced in the single well case. Here, the inversion method used to obtain the KS eigenfunctions and eigenvalues for training sharply turns up towards zero at the edges of our calculation. Counter to that, the predicted potentials vary smoothly towards a constant value with a correct shape of -1/r. If the network were learning for the data-driven difference of potentials, the network would predict this incorrect turning. But, by it's nature the network learns the shape of the decay from the higher density, more information rich, regions of the calculation and continues that trend towards the edges.

% The main struggle of the network for the simpler cases of varying well depth and distance is correctly predicting the cusp of the atomic well. But, we have shown that this problem can be addressed by increasing the resolution of the grid. Creating a trade off between prediction accuracy and training data resolution. While this trade off is useful for understanding the origin of the error in the predicted potentials it may not be feasible to move to obtain extremely fine training data. In this case it might be prudent to employ non-uniform or adaptive grids to generate more points near rapidly varying regions or sharp features in the external potential. While we predict that this would help, the amount that it does compared to increasing the number of points in a uniform grid needs to be researched.

% For the large dataset of varying well depth and distance the error is much less predictable. While this error, similarly to the other cases, will most likely improve with the resolution of the grid it does not originate from there. It is more likely caused by the network construction itself in either the way in which the densities are processed with convolutions, or just the features provided to the dense layers. To address this issue we have looked into predicting XC potentials with neural operators in a data driven context. Further work includes bridging the gap and employing a physics informed neural operator for prediction of XC potentials.

% To learn the physics of the XC potential KS eigenfunctions are necessary. But once the mapping between the XC potential and the electronic density is learned the network can operate without the eigenfunctions. If exact eigenfunctions are provided for the training procedure then the network will learn to predict exact XC potentials and is truly an inversion method rather than an XC approximation. If approximate eigenfunctions are provided then the network will become a learned version of the approximation used to generate said eigenfunctions. This could be useful in testing the networks capabilities when moving into 3D and real systems where highly accurate and exact Ks eigenfunctions are more labor intensive to generate. The networks abilities to learn more accurate XC approximations may provide insight into its usefulness as an inversion scheme for real systems.

% Avoiding the need for KS eigenfunctions would mean moving away from KS DFT and working in orbital free DFT. Here, the effective potential includes a term that relates directly to the electronic density, the pauli potential. 


% The second point is that once these networks are trained they perform inversions much faster than standard inversion methods as seen in Table~\ref{tab:timings_inference}. This point while straightforward is important to bring up. All the test cases presented in this paper are one-dimensional with two particles and while the time to perform an inversion here is palatable it rapidly increases with the number of dimensions, size of the system, and number of particles. Even in this 1D case, the time taken for numerical inversion increases linearly with  charge $z$ and quadratically wrt the grid size while inversion time for the PIML models is constant wrt $z$ and increases linearly with the grid size. With increasing complexity of the system, the time it takes to train the networks might increase but inference time would only depend on the grid size. The efficiency of these PIML models is a significant advantage, particularly in terms of inference speed. The initial investment in training these models is effectively amortized over time, as the substantial time savings during subsequent inversions more than compensates for the upfront cost.



%can be observed in figs \ref{fig:grid_error} and \ref{fig:well_depth_error_501}. For the single well the number of points is increased from 301 to 501 points, by a factor of 1.66, and the peak of the error centered at $x=0$ reduces by about a factor of 1.5. Noticeably, the error on the edges of the grid remain consistent. This reduction in error at the center of the potential results in a significant reduction of eigenvalue error across the range of charge values leaving only the ground state outside the realm of chemical accuracy. This provides a way to systematically improve the error of the network. The bond stretching and full datasets remain on a grid of 301 points for ease of quick computation but should show similar improvement given an increase in the resolution of the data.

%The 1D atomic well is set at zero with two same spin particles. The network is initialized 10 times to to ensure that random initialization is not hiding the network's capabilities. The two particles are to ensure that there is some interaction present and that the network isn't learning just to predict the external potential. The electronic density is computed on a grid spanning a range of [-15,15] of 301 points. $z$ is varied between the values of two and six in steps of 0.1. The final number of data points is 41. %While it would be easy to generate a large amount of training data for this minimal system, the set is kept small in an effort to recreate the common issue of a lack of training data.

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=.8\linewidth]{images/depthxc/eigenvale absolute and log absolute differnce single higher res vertical.png}
%     \caption{MAE (log scaled) of predicted eigenvalues for the same system as the first row of Figure~\ref{fig:all systems diff PINN} but the resolution of the grid is 501 points. The figure also follows the same coloring convention as before. The red horizontal line denotes chemical accuracy.}
%     \label{fig:well_depth_error_501}
% \end{figure}

